Strategies and Challenges of Timestamp Tampering for Improved Digital Forensic Event Reconstruction (extended version)

Timestamps play a pivotal role in digital forensic event reconstruction, but due to their non-essential nature, tampering or manipulation of timestamps is possible by users in multiple ways, even on running systems. This has a significant effect on the reliability of the results from applying a timeline analysis as part of an investigation. In this paper, we investigate the problem of users tampering with timestamps on a running (``live'') system. While prior work has shown that digital evidence tampering is hard, we focus on the question of \emph{why} this is so. By performing a qualitative user study with advanced university students, we observe, for example, a commonly applied multi-step approach in order to deal with second-order traces (traces of traces). We also derive factors that influence the reliability of successful tampering, such as the individual knowledge about temporal traces, and technical restrictions to change them. These insights help to assess the reliability of timestamps from individual artifacts that are relied on for event reconstruction and subsequently reduce the risk of incorrect event reconstruction during investigations.

==> tables/firefox_v_thunderbird.tex <==

\begin{table}[!htb]
    \centering
    \footnotesize
    \begin{tabular}{p{2.5cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
    \toprule
        & \multicolumn{5}{l}{Thunderbird ($n=5$)} && \multicolumn{5}{l}{Firefox ($n=5$)}\\
        \cmidrule(lr){2-6} \cmidrule(lr){8-12}
        Aspects/Participants & 1& 2 & 8 & 9 & 10 && 3 & 4 & 5 & 6 & 7\\
    \midrule
        Conc. inconsistencies & $\bullet$ & & & $\bullet$ & & & $\bullet$ & & $\bullet$ & $\bullet$\\
        Conc. effects & $\bullet$ & & & $\bullet$ & &\\
        Conc. errors & & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & &\\
        Knowledge & & & & & $\bullet$ & & & $\bullet$ & & $\bullet$ & $\bullet$\\
        Effort & $\bullet$ & & & & $\bullet$ & & $\bullet$ \\
        Experience & & & & & & & & & $\bullet$\\
    \bottomrule
    \end{tabular}
    \caption{Aspects driving and influencing the decision-making of each participant, organized per strategy group\todo{useful?}.}
    \label{tab:firefox_vs_thunderbird}
\end{table}




\begin{comment}
\begin{table}[!htb]
    \centering
    \footnotesize
    \begin{tabular}{p{2.5cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
    \toprule
        & \multicolumn{5}{l}{Thunderbird ($n=5$)} && \multicolumn{5}{l}{Firefox ($n=5$)}\\
        \cmidrule(lr){2-6} \cmidrule(lr){8-12}
        Aspects/Participants & 1& 2 & 8 & 9 & 10 && 3 & 4 & 5 & 6 & 7\\
    \midrule
        Conc. inconsistencies & $\bullet$ & & & $\bullet$ & & & $\bullet$ & & $\bullet$ & $\bullet$\\
        Conc. effects & $\bullet$ & & & $\bullet$ & &\\
        Conc. errors & & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & &\\
        Knowledge & & & & & $\bullet$ & & & $\bullet$ & & $\bullet$ & $\bullet$\\
        Effort & $\bullet$ & & & & $\bullet$ & & $\bullet$ \\
        Experience & & & & & & & & & $\bullet$\\
    \bottomrule
    \end{tabular}
    \caption{Aspects driving and influencing the decision-making of each participant, organized per strategy group.}
    \label{tab:firefox_vs_thunderbird}
\end{table}
\end{comment}


==> tables/preparation.tex <==
\begin{table}[!htb]
    \centering
    \footnotesize
    \begin{tabular}{p{2.2cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
    \toprule
        & \multicolumn{5}{c}{Thunderbird} && \multicolumn{5}{c}{Firefox}\\
        \cmidrule(lr){2-6} \cmidrule(lr){8-12}
        Types/Participants & 1& 2 & 8 & 9 & 10 && 3 & 4 & 5 & 6 & 7\\
    \midrule
        AI-based inquiries & &  & $\bullet$ & & & & & $\bullet$\\
        Browser search & & & $\bullet$ & & & & & $\bullet$ & & & $\bullet$\\
        Exploration &$\bullet$ & $\bullet$ & & $\bullet$ &  & & & $\bullet$ & & & $\bullet$\\
        Forums & & & & & & & $\bullet$  & & $\bullet$\\
        Literature review & & & $\bullet$ & & & & & & $\bullet$ & $\bullet$\\
        Testing & $\bullet$ & &  & $\bullet$ & & & $\bullet$ & & $\bullet$ & $\bullet$\\
        Tools review & & $\bullet$ &$\bullet$ & & & & & & $\bullet$ & $\bullet$\\
    \bottomrule
    \end{tabular}
    \caption{Types of preparation steps undertaken by each participant, organized per strategy group.}
    \label{tab:prep}
    %\vspace*{-1.5em}
\end{table}

